A follow-up on intermediate-mass black hole candidates in the second LIGO-Virgo observing run with the Bayes Coherence Ratio

The detection of an intermediate-mass black hole population ($10^2-10^6$ $M_{\odot}$) will provide clues to their formation environments (e.g., disks of active galactic nuclei, globular clusters) and illuminate a potential pathway to produce supermassive black holes. Ground-based gravitational-wave detectors are sensitive to mergers that can form intermediate-mass black holes weighing up to $\sim 450\ M_{\odot}$. However, ground-based detector data contain numerous incoherent short duration noise transients that can mimic the gravitational-wave signals from merging intermediate-mass black holes, limiting the sensitivity of searches. Here we follow-up on binary black hole merger candidates using a ranking statistic that measures the coherence or incoherence of triggers in multiple-detector data. We use this statistic to rank candidate events, initially identified by all-sky search pipelines, with lab-frame total masses $>55\ M_{\odot}$ using data from LIGO's second observing run. Our analysis does not yield evidence for new intermediate-mass black holes. However, we find support for eight stellar-mass binary black holes not reported in the first LIGO-Virgo gravitational wave transient catalog GWTC-1, seven of which have been previously reported by other catalogs.

==> images/bcr_formalism.tex <==

\subsection{Formalism}

Bayes' theorem states that the posterior probability distribution $p(\parameters|d,\mathcal{H})$ for data $d$ and a vector of parameters \parameters that describe a model which quantifies a hypothesis $\mathcal{H}$, is given by
\begin{equation}
p(\parameters|d,\mathcal{H}) = \frac{\mathcal{L}(d|\parameters, \mathcal{H}) \ \pi(\parameters | \mathcal{H})}{\mathcal{Z}(d|\mathcal{H})}\ , 
\end{equation}
where $\mathcal{L}(d|\parameters, \mathcal{H})$ is the likelihood of the data given the parameters \parameters and the hypothesis, $\pi(\parameters | \mathcal{H})$ is the prior probability of the parameters, and finally,
\begin{equation}
    \mathcal{Z}(d|\mathcal{H}) = \int\limits_{\parameters} \ \mathcal{L}(d|\parameters,\mathcal{H}) \ \pi(\parameters | \mathcal{H}) \ d\parameters\ ,
\end{equation} is the likelihood after marginalizing over the parameters \parameters.  To compare two hypotheses $\mathcal{H}_A$ and $\mathcal{H}_B$ through Bayes' theorem one can calculate an odds-ratio
\begin{equation}
    \mathcal{O}^A_B = \frac{\mathcal{Z}^A\ \pi^A}{\mathcal{Z}^B\ \pi^B}\ ,
\end{equation}
where  $\{\pi^A, \pi^B\}$ are the prior-odds for each hypothesis and $\{\mathcal{Z}^A, \mathcal{Z}^B\}$ are shorthand for the evidences $\{\mathcal{Z}(d|\mathcal{H}_A), \mathcal{Z}(d|\mathcal{H}_B)\}$. The odds-ratio can quantify which of the two hypotheses is more likely. For example, if $\mathcal{O}^A_B >> 1$, then the odds are in favor of the $\mathcal{H}_A$ hypotheses. 

The \bcrodds quantity is a Bayesian odds-ratio like the above, of a coherent signal hypotheses $\mathcal{H}_S$ and an incoherent instrumental feature hypothesis $\mathcal{H}_I$ (the null-hypotheses) for a network of $D$ detectors. $\mathcal{H_I}$ states that each detector $i$ has either pure stationary Gaussian noise $\mathcal{H}_N$ or Gaussian noise and an incoherent noise transient (glitch) $\mathcal{H}_G$. Taking $Z^S$, $Z^G_i$ and $Z^N_i$ as the Bayesian evidences (defined in Appendix~\ref{sec:bayesianEvidEval}) for $\mathcal{H}_S$, $\mathcal{H}_N$, and $\mathcal{H}_G$, \bcrodds is given by
\begin{equation}
\label{eq:origbcr}
\bcrodds = \frac{\pi^S Z^S}{\prod\limits^D_{i=1} \ [\pi^G Z^G_i + (1-\pi^G)Z^N_i]}\ ,
\end{equation}

where $\pi^S$ and $\pi^G$ are the prior-odds of obtaining a signal or a glitch from a stretch of data. The prior-odds can be defined more explicitly as 
\begin{itemize}
    \item $\pi^S=\pi(\mathcal{H}_S)/\pi(\mathcal{H}_I)$, the prior-odds for obtaining a coherent signal versus an incoherent instrumental feature.
    \item $\pi^G=\pi(\mathcal{H}_G| \mathcal{H}_I)$, the probability of obtaining a glitch assuming there is an incoherent instrumental feature.
\end{itemize}



When $\mathcal{H}_S$ and $\mathcal{H}_I$ are precisely described and the prior-odds represent our true beliefs, the \bcrodds is a Bayesian odds-ratio. As an odds-ratio, the \bcrodds is the optimal discriminator between coherent signals and incoherent instrumental features. However, as the priors-odds are unknown, we \textit{tune} values for prior-odds, $\hat{\pi}^S$ and $\hat{\pi}^G$, to estimate \bcrodds with a ranking statistic, \bcr, given by
\et{I would remove everything in this subsection before this point. Save it for your dissertation if you want, but I don't think we need to review Bayesian basics here. Instead, just begin by saying that we implement the BCR, which is given by Eq.~\ref{eq:bcr} with suitable references to the previous BCR papers. The motivation for the BCR can be summarised in a single sentence.}
\begin{equation}
\label{eq:bcr}
\bcr = \frac{\hat{\pi}^S Z^S}{\prod\limits^D_{i=1} \ [\hat{\pi}^G Z^G_i + (1-\hat{\pi}^G)Z^N_i]}\ .
\end{equation}
\et{Rewrite the remaining paragraphs to explain that how the BCR relates to the odds with just a few sentences, avoiding equations.}
In the limit where the estimated prior-odds equal the true prior-odds, $\bcr\to\bcrodds$. However, as we are uncertain what the true prior-odds are, it is invalid to use the \bcr as an odds-ratio to make an informed decision about whether a candidate is from an astrophysical or terrestrial source. Instead of interpreting the \bcr as a Bayesian odds-ratio, it can be used as a ranking statistic. Using the \bcr as a ranking statistic we can obtain a frequentist significance of a candidate \bcr-value measured against a background \bcr distribution. 

When using the \bcr as a detection statistic, the prior-odds are empirically tuned to maximize the separation between the \bcr distribution of the background (expected to favor the $\mathcal{H}_I$ hypothesis) and the \bcr distribution of artificially manufactured simulated signals (expected to favor the $\mathcal{H}_S$ hypothesis). Increasing the separation between the two distributions can improve ability of the \bcr to discriminate candidate events as coherent signals or incoherent instrumental features. The tuning process is further described in Appendix~\ref{apdx:tuning-prior-odds}. 



==> titlepage.tex <==


%------ affiliation shortcuts
\newcommand{\SPAno}{School of Physics and Astronomy, Monash University, Clayton VIC 3800, Australia}
\newcommand{\OzGravMonashno}{OzGrav: The ARC Centre of Excellence for Gravitational Wave Discovery, Clayton VIC 3800, Australia}
\newcommand{\CITno}{LIGO Laboratory, California Institute of Technology, Pasadena, CA 91125, USA}
\newcommand{\MITno}{LIGO Laboratory, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\newcommand{\Kavlino}{Department of Physics and Kavli Institute for Astrophysics and Space Research, Massachusetts Institute of Technology, 77 Massachusetts Ave, Cambridge, MA 02139, USA}
\newcommand{\Royal}{Department of Physics, Royal Holloway, University of London, TW20 0EX, United Kingdom}


\title{A search for intermediate-mass black holes mergers in the second LIGO--Virgo observing run with the Bayes Coherence Ratio}


\author{Avi~Vajpeyi} % 0000-0002-4146-1132
\email{avi.vajpeyi@monash.edu}
\affiliation{\SPAno}
\affiliation{\OzGravMonashno}
\author{Rory~Smith} %0000-0001-8516-3324
\affiliation{\SPAno}
\affiliation{\OzGravMonashno}
\author{Eric~Thrane} %0000-0002-4418-3895
\affiliation{\SPAno}
\affiliation{\OzGravMonashno}
\author{Gregory~Ashton} %0000-0001-7288-2231 
\affiliation{\SPAno}
\affiliation{\OzGravMonashno}
\affiliation{\Royal}
\author{Thomas~Alford} % 0000-0003-1942-1334
\affiliation{\CITno}
\author{Sierra~Garza}
\affiliation{\CITno}
\author{Maximiliano~Isi} %0000-0001-8830-8672
\affiliation{\MITno}
\affiliation{\Kavlino}
\author{Jonah~Kanner} % 0000-0001-8115-0577
\affiliation{\CITno}
\author{T. J.~Massinger} %0000-0002-3429-5025
\affiliation{\CITno}
\author{Liting~Xiao} %0000-0003-2703-449X
\affiliation{\CITno}

% \affiliation[\OzGravMonashno]{}
% \affiliation[\MITno]}
% \affiliation[\Kavlino]{}
% \affiliation[\CITno]{}


\date{\today}
